Evaluation of Spectrum Sharing Algorithms for Networks with Heterogeneous Wireless Devices

As highlighted in the National Spectrum Strategy, Dynamic Spectrum Access (DSA) is key for enabling 6G networks to meet the increasing demand for spectrum from various, heterogeneous emerging applications. In this paper, we consider heterogeneous wireless networks with multiple 6G base stations (BS) and a limited number of frequency bands available for transmission. Each BS is associated with a geographical location, a coverage area, and a bandwidth requirement. We assume that clients/UEs are within the corresponding BS's coverage area. To avoid interference, we impose that BSs with overlapping coverage areas must use different frequency bands. We address the challenging problem of efficiently allocating contiguous frequency bands to BSs while avoiding interference. Specifically, we define performance metrics that capture the feasibility of the frequency allocation task, the number of BSs that can be allocated within the limited frequency bands, and the amount of resources utilized by the network. Then, we consider five different DSA algorithms that prioritize BSs based on different features -- one of these algorithms is known in the graph theory literature as Welsh-Powell graph colouring algorithm -- and compare their performance using extensive simulations. Our results show that DSA algorithms that attempt to maximize the chances of obtaining a feasible frequency allocation -- which have been widely studied in the literature -- tend to under-perform in all other metrics.

==> src/algo.tex <==
Description of some of the algorithms and methods for DSA with SCMs, starting with simple cases such as the one used in the SII Demo and moving into more complicated scenarios



\begin{algorithm}
 \caption{Resource sharing between multiple transceivers}
 \begin{algorithmic}[1]
 \STATE \textbf{Input:} \textit{Tx and Rx SCM}\; 
  \STATE \textbf{Output:} \textit{Compatible set of Tx/Rx pairs}\;
  \STATE \textbf{Initialize:} $powerMT = 10$\;
  \STATE \textbf{Initialize:} $interference = \{\}$\;
\FOR{every new set of Tx/Rx pairs}
  \STATE Get its own and existing  Tx/Rx SCMs
    \STATE \textbf{Initialize:} $score = 0$
    \STATE \textbf{Initialize:} $totalTP = 0$
    \STATE \textbf{Initialize:} $maxPM = 0$
    \FOR{ $Rx_n$ check CT btw $Tx_1..Tx_i..Tx_{n-1}$}
    \STATE $totalTP += Tx_iPower$
    \IF{compatible}
    \STATE$score += 1$
     \ENDIF
    \ENDFOR
\STATE $interference[n] = totalTP$
\IF{ $score == n-1$ \textbf{and} $totalTP <= P_{allow Rx_n}$}
\STATE \textbf{Initialize:} $score = 0$
\FOR{ $Tx_n$ check CT btw $Rx_1..Rx_i..Rx_{n-1}$}
\IF{compatible}
    \STATE$score += 1$
     \ENDIF
\STATE $interference[i] += Tx_nPower$  
\STATE $currentPM = interference[i] - P_{allow Rx_i}$
\STATE $maxPM = max(maxPM, currentPM)$
\ENDFOR
\IF{$score == n-1$}
\STATE Setup the new link
\ELSE
\IF{{$maxPM <= powerMT$}}
\STATE \textbf{Adjust} $Tx_n$ reference power
\STATE \textbf{Update} $interference$
\ELSE
\STATE Change $Rx_n$ and $Tx_n$ frequency
\ENDIF
\STATE Setup the new link
\ENDIF
\ELSE
\IF{$score == n-1$ \textbf{and} $totalTP > P_{allow Rx_n}$}
\STATE Detected aggregate interference
\ENDIF
\STATE Change $Rx_n$ and $Tx_n$ frequency
\STATE Setup the new link
\ENDIF
\STATE Update $Rx_n$ and $Tx_n$ SCM
\ENDFOR
 \end{algorithmic}
 \end{algorithm}

==> src/experiment.tex <==
%Description of the setup and results obtained from the SII Demo – very brief (includes a brief description of the COSMOS testbed)
%\cite{stojadinovicspectrum}.
%Our experimentation framework supports and facilitates research of architectures and mechanisms for coordinated use of spectrum resources between collaborative wireless networks. It uses SCMs and was developed on top of the NSF PAWR COSMOS city-scale wireless testbed~\cite{COSMOS_challenge,COSMOS_website,raychaudhuri2005overview}. It aims to enable wireless networks of different domains to exchange messages for coordination in the use of spectrum resources. The framework also facilitates any compatibility computation required to determine available spectrum and avoid interference with other networks using the same spectrum. Figure~\ref{fig:cil_protocol} shows the message types exchanged when a wireless network joins, interacts with other networks, and leaves the service area. The network interaction language for our framework was built on top of DARPA's implementation of CIL. Similar to CIL, each network has a designated wireless domain (WD) controller, which can use the interaction language to communicate with other WDs to coordinate spectrum use. The message types and structure were adapted to make it feasible to transmit SCMs~\cite{scmstandard}. Google Protocol Buffers are used to serialize the messages and their SCM payloads for efficiency. 
\begin{figure}[!b]
\centering
\centerline{\includegraphics[width=\columnwidth]{images/cilprotocol.png}}
\caption{Network Interaction Language protocol detail}
\label{fig:cil_protocol}
%\vspace{-4mm}
\end{figure}
Our experimentation framework supports and facilitates implementation of architectures and mechanisms for coordinated use of spectrum resources between collaborative wireless networks. This framework is built using the ORBIT~\cite{raychaudhuri2005overview} grid within the COSMOS city-scale wireless testbed~\cite{COSMOS_challenge,COSMOS_website}. An important feature of this framework is that it enables wireless networks of different domains to exchange SCMs and perform CTs. % which can be leveraged for coordination in the use of spectrum resources. %The framework also facilitates compatibility computation required to determine available spectrum and avoid interference with other networks using the same spectrum. 
 The network interaction language for our framework was built on top of DARPA's implementation of CIL. Each network has a designated wireless domain (WD) controller, which can use the interaction language to communicate with other networks' WDs. The message types and structure of CIL were adapted to support SCM transmissions~\cite{scmstandard}. Specifically, Fig.~\ref{fig:cil_protocol} shows the message types exchanged when a wireless network joins, interacts with other networks, and leaves the system. The decision-making logic (whether to transmit and which frequency and power to use) of the network is implemented as a part of the WD node logic, and GNU Radio scripts operating on Software Defined Radios (SDRs) are used to implement the functionalities of the transmitter and receiver. Google Protocol Buffers are used to serialize the messages and their SCM payloads for efficiency. The deconfliction of spectrum use takes place automatically via the logic that processed the information of the SCMs and the CTs computations associated with them. For any additional details on the framework and past results we direct readers to our previous work in~\cite{stojadinovicspectrum}.


%We designed several experiments to demonstrate the capabilities of the developed framework. In one of these experiments, we consider three wireless networks, each having a single transmitter-receiver pair in each other's vicinity. The goal is to dynamically reconfigure their wireless transmission characteristics (in particular, their central frequency) so that they become compatible, i.e., there is no harmful interference between devices of different networks. Upon entering the system, all transmitters attempt to use the same spectrum mask and initiate transmission using a 1 MHz wide channel centered at 2000 MHz. The decision-making logic (whether to transmit and which frequency and power to use) of the network is implemented as a part of the WD node logic, and GNU Radio scripts operating on Software Defined Radios (SDRs) are utilized to implement the functionalities of the transmitter and receiver. Fig.~\ref{fig:fosphor} shows the fosphor visualization of the frequency selection of three networks that join the system at times $t_1$, $t_2$, $t_3$. At the end of the experiment, each WD selected a different channel - 2000 MHz, 1999 MHz and 2001 MHz - in order to deconflict the spectrum use and avoid  harmful interference, since no other configuration was found to be feasible. The deconfliction took place automatically via the logic that processed the information of the SCMs and the compatibility computations associated with them.  Table~\ref{tab:parameters} provides our experimentation settings. For  additional details on the framework and results, please see our previous work in~\cite{stojadinovicspectrum}.   

%We designed several experiments to demonstrate the capabilities of the developed framework. In one of the experiments, three wireless networks each having a single transmitter and receiver present in each other's vicinity are considered. The goal is to dynamically reconfigure their wireless transmission characteristics (by changing the central frequency for Tx/Rx operations in our case) so that they become compatible and there is no harmful interference between the devices of different networks. Initially, all transmitters attempt to use the same spectrum mask and initiate transmission using a 1 MHz wide channel centered at 2000 MHz. The decision-making logic (whether to transmit and which frequency and power to use) of the network is implemented as a part of the WD node logic, and GNU Radio scripts operating on Software Defined Radios (SDRs) are utilized to implement the functionalities of transmitter and receiver. Figure~\ref{fig:fosphor} shows the fosphor visualization of three networks joining the domain respectively at time $t_1$, $t_2$, $t_3$ along with their frequency selection. In the end these WDs ended up using three unique channels - 2000 MHz, 1999 MHz and 2001 MHz respectively to deconflict the spectrum use and avoid any harmful interference. The deconfliction took place automatically via the logic that processed the information of the SCMs and the compatibility computations associated with them.  Table~\ref{tab:parameters} provides our experimentation settings and for any additional details on the framework and results we direct readers to please refer to our previous work in ~\cite{stojadinovicspectrum}.   

\comm{\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.32\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/onetx.jpg}
        \caption{One Tx}
        \label{fig:onetx}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/twotx.jpg}
        \caption{Two Tx}
        \label{fig:twotx}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/threetx.jpg}
        \caption{Three TX}
        \label{fig:threetx}
    \end{subfigure}
    \caption{Fosphor visualization showing the spectrum occupancy as the first, second, and third networks start to operate~\cite{stojadinovicspectrum}}
    \label{fig:fosphor}
    \vspace{-2mm}
\end{figure}

\begin{table}[!t]
\centering
\small
\caption{Experimentation Settings}
\begin{tabular}{||l||l|}
\hline
\hline
\textbf{Parameter} & \textbf{Value} \\ \hline
Central Freq       & 2.0 GHz        \\ \hline
No. of Channels    & 3              \\ \hline
Bandwidth    & 1 MHz              \\ \hline
Modulation & BPSK                 \\ \hline
Bitrate & 0.5M                 \\ \hline
Gnuradio & v3.7          \\ \hline    
USRPs & x310s and b210s                 \\ \hline
\end{tabular}
\label{tab:parameters}
\vspace{-4mm}
\end{table}
}

==> src/future.tex <==
%mmwave measurements, reduce complexity of CT, large scale experimentation, ML, open source simulator for future use
In future work, we will consider networks with mmWave nodes using phased array antennas and develop enhanced SCM-based DSA algorithms that take into account antenna directionality. In particular, we plan to: 1) evaluate spectrum utilization for these devices using both the simulator and the COSMOS testbed and 2) develop machine learning-based algorithm tools such as Deep Q-Learning to enable efficient SCM based spectrum access schemes.

%To that end, we will enhance the open source simulator, which currently does not support nodes with directional antennas, and leverage the COSMOS's 
%
%The COSMOS testbed allows for unique mmWave experimentation in a dense urban environment (West Harlem, NYC). We plan to leverage the 
%programmable radios and mmWave phased array antenna modules \cite{gu2021development,chen2021programmable}.

%to evaluate our DSA algorithms in terms of spectrum utilization, power consumption, data throughput, and convergence time. 

==> src/simframework.tex <==

%[Discuss the 50 simulation runs, the random $R_i$ and $B_i$, and the base parameters.]
To evaluate the performance of our sorting methods, we use an object-oriented, Python-based simulator based on Monte-Carlo methods to run proposed algorithms and model geographic and spectral deployment of transmitters. The simulator models our heterogeneous network environment, applies our sorting and allocation strategies from Section 3 and 4, and evaluates each sorting method’s performance with respect to our objective functions, as defined in Section 2. Ultimately, the simulator employs an event-based framework in which transmitters join the system sequentially. To ensure accurate results, the data is averaged over 50 randomized trials, providing a statistically significant analysis of performance variations. The default simulation parameters and computational resources are summarized in table X. 

\begin{table}[!h]
\centering
\small
\vspace{-2mm}
\caption{Simulation Parameters}
\begin{tabular}{lc}%||l||l|
%\hline
%\hline
\toprule
\textbf{Parameter} & \textbf{Value} \\ \midrule %\hline
%Latitude (min, max)      & (40.805726, 40.812829)\\
%Longitude (min, max)      & (-73.945219, -73.955432)\\
Geographical Area&   $100\times100 m^2$\\ %\hline
Number of Transmitters&  $N=$ 25 \\ %\hline
Total Available Bandwidth&  $F=$ 10 units\\ %\hline
Bandwidth of Transmitter $i$&   $B_i \sim Uniform(1, 3)$\\ %\hline
Coverage of Transmitter $i$&   $R_i \sim Uniform(8, 17)$\\ %\hline
Number of Simulation Runs&  $50$\\ %\hline
\bottomrule
\end{tabular}
\label{tab:sim_parameters}
\vspace{-4mm}
\end{table}

% The simulator assigns ordered lists of transmitters into the spectrum based on the selected sorting and allocation algorithms. Each simulation run includes a set of randomly generated transmitters characterized by their geographic coordinates, signal propagation radius, and bandwidth requirements, which are all selected uniformly at random. The geographic coordinates are between 0 and 100 meters to position each node within the 100 by 100 square meter area. We constrain the transmit power such that the coverage radius for each transmitter is between 8 and 17 meters inclusive. Transmitter bandwidth requests are between 1 and 3 units inclusive. Moreover, we default spectral bandwidth to 10 units and the number of transmitters in the system to a count of 25. In the subsequent section, we discuss the results derived from these simulations in the form of line graphs.
The simulator assigns ordered lists of transmitters into the spectrum based on the selected sorting and allocation algorithms. Each simulation run includes a set of randomly generated transmitters characterized by their geographic coordinates, signal propagation radius, and bandwidth requirements, which are all selected uniformly at random. The geographic coordinates \((x_i, y_i)\) for each transmitter \(T_i\) are selected such that \(0 \leq x_i, y_i \leq 100\) meters, positioning each node within the \(100 \times 100\) square meter area. We constrain the transmit power such that the coverage radius \(R_i\) for each transmitter \(T_i\) is between 8m and 17m inclusive, i.e., \(8 \leq R_i \leq 17\) meters. Transmitter bandwidth requests \(B_i\) are between 1 and 3 units inclusive, i.e., \(1 \leq B_i \leq 3\) units. Moreover, we default the spectral bandwidth \(B_{total}\) to 10 units and the number of transmitters \(T_x\) in the system to a count of 25. In the subsequent section, we discuss the results derived from these simulations in the form of line graphs.


==> src/simulation.tex <==
%Results from simulations that use SCMs to deconflict spectrum use between a large number of devices.
%Focus on performance measures related to spectrum use: How many channels to deconflict spectrum use. Mention that future work will try to reduce the number of channels further but the declarative nature of SCMs is a key asset to the process.
In this section, we develop and evaluate an enhanced SCM-based DSA algorithm that can be used to deconflict the spectrum use of networks with a large number of devices. The algorithm proposed in Section~\ref{algo}, below, leverages CIL and SCMs to dynamically configure the transmission parameters of RF devices, in particular their central frequency and transmission power levels, in order to achieve aggregate compatibility. %Additional details about the algorithm are discussed in Section~\ref{algo}. 
To evaluate the performance of this algorithm, we use a custom-designed simulation platform. In Section~\ref{platform} and ~\ref{results}, we describe the simulation platform and the results respectively. 
%The experiment described in Section~\ref{experiment} involved three networks and employed a relatively simple algorithm to coordinate the spectrum use. Taking this as a baseline, in this work we developed a more complex algorithm that uses SCMs to deconflict spectrum use between a large number of devices. The algorithm considers aggregate interference along with the option of limiting the transmission power of any new transmitter joining the system for efficient utilization of available spectrum. More details on the algorithm can be found below including simulation results in Section \ref{result}.

% \begin{algorithm}[!b]
% \small
% \SetAlgoLined 
% \textbf{Input:} \textit{SCMs of new and existing Tx/Rx pairs}\\ 
% \textbf{Output:} \textit{Deconflicted Tx/Rx pairs}\\
% \textbf{Initialize:} $power_{MT}$\\
% \textbf{Initialize:} $Rx_{interf} = [\ ]$\\
% \For{every new set of $Tx/Rx$ pairs}
% {
% Get its own and existing  $Tx/Rx$ SCMs\\
% \textbf{Initialize:} $ct\_score = 0$\\
% \textbf{Initialize:} $total_{TP} = 0$\\
% \textbf{Initialize:} $max_{PM} = 0$\\
% \For{$Rx_n$ check C.T. $btw$ $Tx_1..Tx_i..Tx_{n-1}$}
% {
% $total_{TP} += Tx_{inPower}$\\
% \If{\textit{compatible}}
% {
% $ct\_score += 1$
% }
% }
% \If{$ct\_score == n-1$ \textbf{and} $total_{TP} <= P_{allow Rx_n}$}
% {
% \textbf{Initialize:} $ct\_score = 0$\\
% $Rx_{interf}[n] = total_{TP}$\\
% $Tx_n\_interf = [ \ ]$\\
% \For{ $Tx_n$ check C.T. $btw$ $Rx_1..Rx_j..Rx_{n-1}$}
% {

% $Tx_n\_interf[j] = Tx_{njPower}$\\ 
% $current_{PM} = Rx_{interf}[j]+Tx_{njPower} - P_{allow Rx_j}$\\
% $max_{PM} = max(max_{PM}, current_{PM})$

% \If{\textit{compatible} \textbf{and} $current_{PM} <=0$}
% {
% $ct\_score += 1$
% }
% }
% \If{$ct\_score == n-1$}
% {
% \textbf{Update} $Rx_{interf} += Tx_n\_interf$
% }
% \Else{
% \If{$max_{PM} <= power_{MT}$}
% {
% \textbf{Adjust} $Tx_n$ reference power based on $max_{PM}$\\
% \textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Tx_n\_interf$

% \textbf{Verify} if the new link is reachable or not.
% }
% \Else{
% \textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
% }
% }
% }
% \Else{
% \If{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
% {
% Aggregate interference detected
% }
% \textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
% }
% Setup the new link\\
% Update $Rx_n$ and $Tx_n$ SCM
% }
% \caption{Spectrum Deconfliction (SD)} \label{algo:1}
% \end{algorithm}

\begin{algorithm}[!b]
\small
\SetAlgoLined 
\textbf{Input:} \textit{SCMs of new and existing Tx/Rx pairs}\\ 
\textbf{Output:} \textit{Deconflicted Tx/Rx pairs}\\
\textbf{Initialize:} $power_{MT}$ and $Rx_{interf} = [\ ]$\\
\For{every new set of $Tx/Rx$ pairs}
{
Collect own and existing $Tx/Rx$ SCMs\\
\textbf{Initialize:} $ct\_score = 0$, $total_{TP} = 0$ and $max_{PM} = 0$\\
\For{$Rx_n$ check C.T. $btw$ $Tx_1..Tx_i..Tx_{n-1}$}
{
$total_{TP} += Tx_{inPower}$\\
\If{\textit{compatible}}
{
$ct\_score += 1$
}
}
\If{$ct\_score == n-1$ \textbf{and} $total_{TP} <= P_{allow Rx_n}$}
{
\textbf{Initialize:} $ct\_score = 0$\\
$Rx_{interf}[n] = total_{TP}$\\
$Tx_n\_interf = [ \ ]$\\
\For{ $Tx_n$ check C.T. $btw$ $Rx_1..Rx_j..Rx_{n-1}$}
{

$Tx_n\_interf[j] = Tx_{njPower}$\\ 
$current_{PM} = Rx_{interf}[j]+Tx_{njPower} - P_{allow Rx_j}$\\
$max_{PM} = max(max_{PM}, current_{PM})$

\If{\textit{compatible} \textbf{and} $current_{PM} <=0$}
{
$ct\_score += 1$
}
}
\If{$ct\_score == n-1$}
{
\textbf{Update} $Rx_{interf} += Tx_n\_interf$
}
\Else{
\If{$max_{PM} <= power_{MT}$}
{
\textbf{Adjust} $Tx_n$ reference power based on $max_{PM}$\\
\textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Tx_n\_interf$

\textbf{Verify} if the new link is reachable or not.
}
\Else{
\textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
}
}
}
\Else{
\If{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
{
Aggregate interference detected
}
\textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
}
Setup the new link\\
Update $Rx_n$ and $Tx_n$ SCM
}
\caption{Spectrum Deconfliction (SD)} \label{algo:1}
\end{algorithm}

\subsection{Algorithm for DSA with SCMs}\label{algo}
The deconfliction of spectrum use for networks with a large number of RF devices is based on the computation of aggregate interference %mainly involves compatibility computations 
between new and existing devices. %in a peer-to-peer fashion. 
 To this end, we propose a novel SCM-based Spectrum Deconfliction (SD) method as described in Algorithm~\ref{algo:1} with key terms defined in Table~\ref{tab:terminology}. In particular, when a new pair of devices ($Tx_n$ and $Rx_n$) enters an operational area, the SD algorithm running at the corresponding WD controller requests the SCMs of new and existing $Tx$ and $Rx$ pairs and then it initializes the following parameters: compatibility score ($ct\_score=0$), total power margin ($total_{PM}=0$) and max power margin ($max_{PM}=0$). The score is used to verify the compatibility of the new Tx/Rx pair with the entire system whereas the power margins are used to verify whether small adjustments in the power level %used in cases where we can determine that a small adjustment to the power 
of the new transmitter ($Tx_n$) can make it compatible with the existing receivers. 
\par Next, the WD controller performs compatibility tests, as described in Section~\ref{compatibility_test}, between the new $Rx_n$ and existing transmitters ($Tx_1...Tx_{n-1}$). Based on the test results, the WD controller updates the score and obtains the total aggregate interference ($total_{TP}$) at $Rx_n$. If $Rx_n$ is not compatible with the existing transmitters or if the $total_{TP}$ is greater than the allowable interference power at $Rx_n$ (identified as $P_{allow Rx_n}$), the Tx and Rx pair are moved to a different frequency/channel and the compatibility tests start over (more details on the frequency assignment scheme will be discussed later). Finally, if $Rx_n$ is compatible with the existing transmitters, the WD controller verifies whether $Tx_n$ is compatible with the existing receivers ($Rx_1...Rx_{n-1}$). To that end, it computes the interference caused by $Tx_n$ at the existing receivers and compares it with $max_{PM}$. If $Tx_n$ is compatible with the receivers already operating in the operational area, the WD controller sets up the new link and updates the contribution of this new transmitter to the aggregate interference seen by each receiver using the matrix ($Rx_{interf}$). Otherwise, the WD controller tries to achieve compatibility by decreasing $Tx_n$'s power by no more than the value of the power margin threshold ($power_{MT}$). In case power adjustment fails to achieve compatibility, the WD controller chooses a different frequency channel for the Tx and Rx pair and the compatibility tests start over. At the end of the algorithm, once aggregate compatibility is achieved, the WD controller sets up the link and updates both $Tx_n$ and $Rx_n$ SCMs based on their corresponding frequency and power usage so that they are ready for any future compatibility computations. %The complete procedure is described in Algorithm~\ref{algo:1} with key terms defined in Table~\ref{tab:terminology}.

Regarding frequency assignment, upon entering the operational area, all RF devices start with a default center frequency of 2000 MHz and then move to a new frequency in 1 MHz increments whenever needed, based on the results of the compatibility computations, until a compatible frequency for the operation of the Tx/Rx pair is found. In doing so, the objective here is to achieve high spectrum efficiency with minimum usage of frequency channels. 



% \iffalse
% \begin{algorithm}
%  \caption{Spectrum Deconfliction (SD) Mechanism}
%  \label{algo:1}
%  \begin{algorithmic}[1]
%  \State \textbf{Input:} \textit{SCMs of new and existing Tx/Rx pairs} 
%   \State \textbf{Output:} \textit{Deconflicted Tx/Rx pairs}
%   \State \textbf{Initialize:} $power_{MT}$
%   \State \textbf{Initialize:} $Rx_{interf} = [\ ]$
% \For{every new set of $Tx/Rx$ pairs}
%   \State Get its own and existing  $Tx/Rx$ SCMs
%     \State \textbf{Initialize:} $ct\_score = 0$
%     \State \textbf{Initialize:} $total_{TP} = 0$
%     \State \textbf{Initialize:} $max_{PM} = 0$
%     \For{$Rx_n$ check C.T. $btw$ $Tx_1..Tx_i..Tx_{n-1}$}
%     \State $total_{TP} += Tx_{inPower}$
%     \If{\textit{compatible}}
%     \State$ct\_score += 1$
%      \EndIf
%     \EndFor
% \If{$ct\_score == n-1$ \textbf{and} $total_{TP} <= P_{allow Rx_n}$}
% \State \textbf{Initialize:} $ct\_score = 0$
% \State $Rx_{interf}[n] = total_{TP}$
% \State $Tx_n\_interf = [ \ ]$
% \For{ $Tx_n$ check C.T. $btw$ $Rx_1..Rx_j..Rx_{n-1}$}
% \If{\textit{compatible}}
%     \State$ct\_score += 1$
%      \EndIf
%     \State $Tx_n\_interf[j] = Tx_{njPower}$ 
% \State $current_{PM} = $ \\ $Rx_{interf}[j]+Tx_{njPower} - P_{allow Rx_j}$
% \State $max_{PM} = max(max_{PM}, current_{PM})$
% \EndFor
% \If{$ct\_score == n-1$}
% \State \textbf{Update} $Rx_{interf} += Tx_n\_interf$
% \Else
% \If{{$max_{PM} <= power_{MT}$}}
% \State \textbf{Adjust} $Tx_n$ reference power based on $max_{PM}$
% \State \textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Tx_n\_interf$
% \Else
% \State \textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
% \EndIf
% \EndIf
% \Else
% \If{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
% \State Aggregate interference detected
% \EndIf
% \State \textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
% \EndIf
% \State Setup the new link
% \State Update $Rx_n$ and $Tx_n$ SCM
% \EndFor
%  \end{algorithmic}
%  \end{algorithm}
% \fi

% %\iffalse
% \begin{algorithm}
%  \caption{Spectrum Deconfliction (SD)}
%  \label{algo:1}
%  \begin{algorithmic}[1]
%  \STATE \textbf{Input:} \textit{SCMs of new and existing Tx/Rx pairs}\; 
%   \STATE \textbf{Output:} \textit{Deconflicted Tx/Rx pairs}\;
%   \STATE \textbf{Initialize:} $power_{MT}$\;
%   \STATE \textbf{Initialize:} $Rx_{interf} = [\ ]$\;
% \FOR{every new set of $Tx/Rx$ pairs}
%   \STATE Get its own and existing  $Tx/Rx$ SCMs
%     \STATE \textbf{Initialize:} $ct\_score = 0$
%     \STATE \textbf{Initialize:} $total_{TP} = 0$
%     \STATE \textbf{Initialize:} $max_{PM} = 0$
%     \FOR{$Rx_n$ check C.T. $btw$ $Tx_1..Tx_i..Tx_{n-1}$}
%     \STATE $total_{TP} += Tx_{inPower}$
%     \IF{\textit{compatible}}
%     \STATE$ct\_score += 1$
%      \ENDIF
%     \ENDFOR
% \IF{$ct\_score == n-1$ \textbf{and} $total_{TP} <= P_{allow Rx_n}$}
% \STATE \textbf{Initialize:} $ct\_score = 0$
% \STATE $Rx_{interf}[n] = total_{TP}$
% \STATE $Tx_n\_interf = [ \ ]$
% \FOR{ $Tx_n$ check C.T. $btw$ $Rx_1..Rx_j..Rx_{n-1}$}
% \IF{\textit{compatible}}
%     \STATE$ct\_score += 1$
%      \ENDIF
%     \STATE $Tx_n\_interf[j] = Tx_{njPower}$ 
% \STATE $current_{PM} = $ \\ $Rx_{interf}[j]+Tx_{njPower} - P_{allow Rx_j}$
% \STATE $max_{PM} = max(max_{PM}, current_{PM})$
% \ENDFOR
% \IF{$ct\_score == n-1$}
% \STATE \textbf{Update} $Rx_{interf} += Tx_n\_interf$
% \ELSE
% \IF{{$max_{PM} <= power_{MT}$}}
% \STATE \textbf{Adjust} $Tx_n$ reference power based on $max_{PM}$
% \STATE \textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Tx_n\_interf$
% \ELSE
% \STATE \textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
% \ENDIF
% \ENDIF
% \ELSE
% \IF{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
% \STATE Aggregate interference detected
% \ENDIF
% \STATE \textbf{Change} $Rx_n$ and $Tx_n$ \underline{frequency} and recompute compatibility tests
% \ENDIF
% \STATE Setup the new link
% \STATE Update $Rx_n$ and $Tx_n$ SCM
% \ENDFOR
%  \end{algorithmic}
%  \end{algorithm}
% %\fi
 
\subsection{Simulation Platform}\label{platform}
To evaluate the performance of our proposed SD algorithm, we use a Python-based simulator that assigns transmitter-receiver pairs to random locations on a given operational area and then uses the procedures described in Algorithm \ref{algo:1} to deconflict the spectrum use. The simulation uses a Simpy event-based framework with transmitter-receiver pairs joining the system sequentially, i.e., one after the other. The simulation parameters are summarized in Table~\ref{tab:sim_parameters}. To perform compatibility tests, we leverage Octave code from the Spectrum Consumption Model Builder and Analysis Tool (SCMBAT)~\cite{SCMBAT_website} which interfaces our python simulator using \textit{oct2py}. The SCMs used in the simulator are similar to the SCMs from our prior experimental work in~\cite{stojadinovicspectrum}, except that, now we are limiting the transmit power such that the coverage radius is around 100 meters. The structure of the transmitter spectrum mask and receiver underlay mask are illustrated in Fig.~\ref{fig:tx_rx_masks}. The position of the transmitters are chosen uniformly at random in a 0.5 square mile area, subject to the constraint of a minimum distance of 10 meters between any two transmitters. Moreover, the separation between a transmitter and the associated receiver is chosen uniformly at random in the interval between 10 and 100 meters. Next, for a scenario involving large number of RF devices, we discuss the simulation results of our SD algorithm against a \emph{baseline} algorithm that only adjusts center frequencies to deconflict spectrum use, in terms of its computation time and spectrum resource usage.

\begin{table}[h]
\centering
\small
\caption{Key Parameters of Algorithm~\ref{algo:1}}
\begin{tabular}{||l||l|}
\hline
\hline
\textbf{Parameter} & \textbf{Description} \\ \hline
$Tx_{ijPower}$    & \begin{tabular}[c]{@{}l@{}}Interference power at j\textsuperscript{th} receiver from i\textsuperscript{th} \\ transmitter \end{tabular}          \\ \hline
$Rx_{interf}$    & \begin{tabular}[c]{@{}l@{}}Interference at each $Rx$ from all \\ existing $Txs$ (vector) \end{tabular}          \\ \hline
$Tx_n\_{interf}$ & \begin{tabular}[c]{@{}l@{}}Interference at each $Rx$ from \\ $Tx_n$ (vector) \end{tabular}  \\ \hline
$total_{TP}$    & \begin{tabular}[c]{@{}l@{}}Total transmit power at $Rx_n$ from \\ all existing $Txs$ (interference) \end{tabular}\\ \hline
$power_{MT}$       & Power margin threshold        \\ \hline
$max_{PM}$ & Max power margin from all $Rxs$                 \\ \hline
$current_{PM}$ & Current power margin          \\ \hline    
$P_{allow Rx_n}$ & Allowable power at $Rx_n$                \\ \hline
$C.T.$ & Compatibility Test                \\ \hline
\end{tabular}
\label{tab:terminology}
\end{table}

\begin{figure}[h]
  \vspace{-3mm}
  \centering
  \begin{subfigure}[t]{0.24\textwidth}
    \centering

    \includegraphics[width=1\linewidth]{images/icc-tx.png}
    \caption{ }
  \end{subfigure}
  \begin{subfigure}[t]{0.24\textwidth}
    \centering

    \includegraphics[width=1\linewidth]{images/icc-rx.png}
    \caption{ }
  \end{subfigure}
  \caption{(a) TX spectrum mask. (b) RX underlay mask.}\label{fig:tx_rx_masks} 
  \vspace{-3mm}
\end{figure}

\subsection{Simulation Results}\label{results}
\subsubsection{Computation time}
We evaluate the time required by Algorithm~\ref{algo:1}, which takes into account aggregate interference effects and adjusts both center frequencies and Tx power levels based on compatibility tests, against a \emph{baseline algorithm} to deconflict the spectrum use i.e., the time to determine a compatible set of parameters for every transmitter-receiver pair in the operational area. %Tx and Rx devices that are part of a Tx/Rx link pair so that they are compatible with all previous Tx/Rx link pairs. 
%Recall that pairs join the system sequentially. Hence, 
The computation time does not include: (i) pauses between new link pair instances (recall that pairs join the system sequentially); (ii) time to turn on the RF devices, which depends on the radios being used; nor (iii) SCM transmission times, which usually take a few milliseconds. For each simulation setup, 100  trials/runs are executed. Fig.~\ref{fig:convergence_time} shows the mean computation time for networks with different numbers of transmitter-receiver pairs. We observe that to configure a single new link in a scenario composed of 20 pre-existing links the SD algorithm takes (on average) 0.39 seconds as compared to the 5.6 seconds required in a scenario with 100 pre-existing link-pairs. The increase in convergence time with the increase in the total number of transmitter-receiver pairs is expected and it is mainly due to the larger number of aggregate compatibility tests that need to be performed. To setup a single new link in a scenario that already has 100 operational link-pairs, the baseline algorithm takes (on average) 3.51 seconds. The lower computation time for the baseline scheme is due to the lower number of compatibility tests being performed, since it mainly processes frequency changes without performing additional link reachability tests as in Algorithm~\ref{algo:1}. The convergence time can be significantly reduced by using more powerful CPUs and also by further optimizing the algorithm.
%Considering that the algorithm takes into account the impact of aggregate interference, Tx power calibration and compatible frequency/channel allocation, it converges well within a finite amount of time for a large number of links. The convergence time depends heavily on the characteristics of the system that is doing the compatibility computations and can be scaled down considerably with the use of high end machines. The increase in convergence time with the increase in number of links is expected as it's mainly due to the higher number of compatibility evaluations present as the number of devices grows. Further optimization to the algorithm are left for future work.
\begin{table}[!h]
\centering
\small
\caption{Simulation Parameters}
\begin{tabular}{||l||l|}
\hline
\hline
\textbf{Parameter} & \textbf{Value} \\ \hline
Latitude      & \begin{tabular}[c]{@{}l@{}}\textbf{Min:} 40.805726\\ \textbf{Max:} 40.812829 \end{tabular}       \\ \hline
Longitude      & \begin{tabular}[c]{@{}l@{}}\textbf{Min:} -73.945219\\ \textbf{Max:} -73.955432 \end{tabular}       \\ \hline
Operational Area       &   0.5 square mile     \\ \hline
Min Tx-Tx separation       &   10 m     \\ \hline
Tx-Rx separation       &   $Uniform(10m, 100m)$    \\ \hline
Frequency shift       &   1 MHz     \\ \hline
Power margin threshold      &   3 dB     \\ \hline
Number of trials      &  100     \\ \hline
Python version       &   3.8    \\ \hline
Machine configuration      &  \begin{tabular}[c]{@{}l@{}}Intel i7-4790 (3.60 GHz)\\ Cores: 8, Memory: 15 GB \end{tabular}     \\ \hline
\end{tabular}
\label{tab:sim_parameters}
%\vspace{-6mm}
\end{table}

\begin{figure}[h]
\vspace{-8mm}
\centering
\centerline{\includegraphics[width=0.9\columnwidth]{images/computation_time.png}}
\caption{Average time required per link by the SD and baseline algorithms to deconflict spectrum use}
\label{fig:convergence_time}
\vspace{-4mm}
\end{figure}

\subsubsection{Spectrum usage}
We evaluate the spectrum usage of Algorithm~\ref{algo:1} considering the number of frequency channels used and Tx power adjustments. As shown in Fig.~\ref{fig:resource_freq}, for 100 trials, the maximum number of channels required to configure 10 links is 5 as compared to 9 channels required to configure 100 links. The mode number of channels required for 10, 50 and 100 links are 2, 6 and 6, respectively. We also observe that, to support a large number of links (100 in our case), we require only a few channels (max 9 channels) and it is mainly due to the Tx reference power adjustment as shown in Table~\ref{tab:performance_cnt}. We limit the transmit power of new transmitters based on the power margin threshold and power margin obtained from the compatibility tests. If a compatibility computation indicates that the Tx power of a transmitter if reduced by an amount that does not exceed the value indicated by the power margin threshold will lead to compatibility with all previous receivers, the adjustment is applied, otherwise the transmitter will need to move to a different frequency/channel. The average number of Tx reference power adjustments for 10 and 100 links over 100 trials is found to be 1.19 and 13.54, respectively. For scenarios with a large number of links, sometimes when trying to execute the power adjustment step, it leads to a transmitter not being able to reach its intended receiver. This forces the use of a different frequency channel for the Tx/Rx pair and the need to perform compatibility tests again. The average non reachable link count events for 100 links over 100 trials is found to be 265.75, thus requiring higher computation time to deconflict the spectrum in the network as observed in Fig.~\ref{fig:convergence_time}.

%\begin{figure*}[ht]%
%\centering
%\begin{subfigure}{0.65\columnwidth}
%\begin{center}
%\includegraphics[width=1.\linewidth]{images/resource_frequency.png}%
%\caption{\label{fig:resource_freq}Histogram depicting channel \\allocation %for multiple link configuration}
%\end{center}
%\end{subfigure}
%\begin{subfigure}{0.65\columnwidth}
%\begin{center}
%\includegraphics[width=1.\linewidth]{images/resource_power_cnt.png}%
%\caption{\label{fig:resource_pow} Histogram of Tx power adjustment %\\counter for multiple link configuration.}
%\end{center}
%\end{subfigure}%
%%\newline
%\begin{subfigure}{0.65\columnwidth}
%%\begin{center}
%\includegraphics[width=1.\linewidth]{images/dsa_schemes.png}%
%\caption{\label{fig:result_dsa_scheme}Histogram showing channel allocation %for two DSA schemes having 100 links.}
%%\end{center}
%\end{subfigure}
%\caption{\label{sim-res} DSA with SCMs simulation results}
%\end{figure*}

\begin{figure}[h]
\vspace{-4mm}
\centering
\centerline{\includegraphics[width=0.9\columnwidth]{images/resource_frequency.png}}
\caption{Histogram depicting channel allocation of Algorithm~\ref{algo:1} for multiple link configuration and 100 random trials.}
\label{fig:resource_freq}
\vspace{-4mm}
\end{figure}


%\begin{figure}[t]
%\centering
%\centerline{\includegraphics[width=0.95\columnwidth]{images/resource_power_cnt.png}}
%\caption{Histogram showing Tx power adjustment counter for different number of links and trials.}
%\label{fig:resource_pow}
%\vspace{-4mm}
%\end{figure}

\subsubsection{Performance comparison} We compare the spectrum usage of Algorithm~\ref{algo:1} and the baseline algorithm considering 100 links over 100 unique trials. %Two different DSA schemes were evaluated considering the same simulation setup. For the baseline case, we only 
%considered frequency assignment decisions based on compatibility tests with no other adaptation to RF operational parameters. 
In Fig.~\ref{fig:result_dsa_scheme}, %shows that our proposed SD method (Algorithm~\ref{algo:1}) performs fairly well as compared to the baseline algorithm %.
when looking at the mode number values,  about two times more channels are required for the baseline case as compared to our proposed scheme, since the baseline algorithm just operates on assigning frequencies of operation without adapting Tx power levels. The other important metric in the evaluation is the presence of aggregate interference in the system. We defined a counter for aggregate interference events that is incremented was found to be not compatible when taking into account the interference caused by all existing transmitters event though it was compatible with the transmitters on a one to one basis. Table~\ref{tab:agg_interference} provides the number of times (cases) that aggregate interference effects led to an incompatibility decision in 100 runs/trials. In each of those cases, the device would need to move to a different frequency to be protected from aggregate interference effects. The results obtained indicate that as the number of devices grows, the effects of aggregate interference and adjacent channel power leakage are well captured with the use of SCMs.  A higher aggregate interference is observed for the baseline as compared to Algorithm~\ref{algo:1}, due to the presence of large number of channels being used without any power adjustments causing higher adjacent channel interference. Moreover, the aggregate interference highly depends on the Tx/Rx location coordinates and channels being used.

\begin{table}[t]
%\vspace{-2mm}
\centering
\small
\caption{Performance counters of Algorithm 1 averaged over 100 trials for different link configurations}
\begin{tabular}{||c||l|l|l|l|l|}
\hline
\hline
\textbf{Links}                                                            & \textbf{10} & \textbf{20} & \textbf{50} & \textbf{80} & \textbf{100} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Avg. \# of power\\ adjustments \end{tabular}} & 1.19 & 5.97 & 14.19 & 13.67 & 13.54 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Avg. \# of non-\\reachable events\end{tabular}} & 0.19 & 2.53 & 71.39 & 190 & 265.75 \\ \hline
\end{tabular}
\label{tab:performance_cnt}
\vspace{-2mm}
\end{table}

\begin{table}[t]
%\vspace{-2mm}
\centering
\small
\caption{Presence of aggregate interference averaged over 100 trials for different link configurations}
\begin{tabular}{||c||l|l|l|l|l|}
\hline
\hline
\textbf{Links}                                                            & \textbf{10} & \textbf{20} & \textbf{50} & \textbf{80} & \textbf{100} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Baseline\end{tabular}} & 0.13 & 0.64 & 6.63 & 20.94 & 32.99 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Algorithm 1\end{tabular}} & 0.11 & 0.53 & 1.19 & 1.52 & 1.44 \\ \hline
\end{tabular}
\label{tab:agg_interference}
\vspace{-4mm}
\end{table}
%avg channel used

\begin{figure}[h]
\vspace{-5mm}
\centering
\centerline{\includegraphics[width=0.9\columnwidth]{images/dsa_schemes.png}}
\caption{Histogram for number of channels used - baseline vs. SD Algorithm (100 links \& 100 trials).}
\label{fig:result_dsa_scheme}
\vspace{-4mm}
\end{figure}

\begin{table*}[ht]
\centering
\small
\caption{\label{tab:comp_error}Compatibility error (\%) and Avg. computation time per link (C.T. in seconds) due to \textbf{SD optimization}, averaged over 30 random trials in networks of different sizes.}
\begin{tabular}{||c||cc|cc|cc|cc|cc|}
\hline\hline 
\textbf{Links}                                                                                                    & \multicolumn{2}{c|}{\textbf{10}}               & \multicolumn{2}{c|}{\textbf{20}}               & \multicolumn{2}{c|}{\textbf{50}}               & \multicolumn{2}{c|}{\textbf{80}}               & \multicolumn{2}{c|}{\textbf{100}}              \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}} Error in \% \&\\ C.T. in seconds  \end{tabular}} & \multicolumn{1}{l|}{\textbf{\%}} & \textbf{sec} & \multicolumn{1}{l|}{\textbf{\%}} & \textbf{sec} & \multicolumn{1}{l|}{\textbf{\%}} & \textbf{sec} & \multicolumn{1}{l|}{\textbf{\%}} & \textbf{sec} & \multicolumn{1}{l|}{\textbf{\%}} & \textbf{sec} \\ \hline 
\textbf{D = 100m}                                                                                                 & \multicolumn{1}{l|}{10}          & 0.010       & \multicolumn{1}{l|}{13}          & 0.020       & \multicolumn{1}{l|}{1.8}         & 0.054       & \multicolumn{1}{l|}{0.16}        & 0.088       & \multicolumn{1}{l|}{0}           & 0.106       \\ \hline
\textbf{D = 200m}                                                                                                 & \multicolumn{1}{l|}{1.33}        & 0.025       & \multicolumn{1}{l|}{0.33}        & 0.053       & \multicolumn{1}{l|}{0}           & 0.173       & \multicolumn{1}{l|}{0}           & 0.309       & \multicolumn{1}{l|}{0}           & 0.396       \\ \hline
\textbf{D = 300m}                                                                                                 & \multicolumn{1}{l|}{0.6}        & 0.047       & \multicolumn{1}{l|}{0}            & 0.100       & \multicolumn{1}{l|}{0}           & 0.377       & \multicolumn{1}{l|}{0}           & 0.736       & \multicolumn{1}{l|}{0}           & 1.055       \\ \hline
\textbf{D = 500m}                                                                                                 & \multicolumn{1}{l|}{0.6}         & 0.085       & \multicolumn{1}{l|}{0}           & 0.212       & \multicolumn{1}{l|}{0}           & 0.95        & \multicolumn{1}{l|}{0}           & 1.97        & \multicolumn{1}{l|}{0}           & 2.57        \\ \hline 
\end{tabular}
\vspace{-4mm}
\end{table*}

\subsubsection{SD algorithm optimization} Finally, we evaluate the performance effects on the spectrum deconfliction algorithm by introducing a distance parameter (D), where we only perform compatibility tests against the devices that are within a distance threshold of D rather than with all existing devices. When setting D=100m or D=300m, the computation time is significantly reduced as compared to the exhaustive case. As an example, having 100 links, the average computation time for D=100m and D=300m is found be 0.106s and 1.055s respectively as compared to 5.59s required for Algorithm~\ref{algo:1} (see Table~\ref{tab:comp_error}) without any optimization. For D=500m, the spectrum usage and the impact of aggregate interference is similar to the exhaustive solution (Algorithm~\ref{algo:1}, see Fig.~\ref{fig:sd_opt_freq}), implying that for up to 500m, the aggregate interference from existing devices is impacting the new device and is well captured with the help of SCMs. Sometimes, these optimizations with distances lead to compatibility errors and we compute this error with respect to the exhaustive case where the evaluation of compatibility is done agains all existing devices as shown in Table~\ref{tab:comp_error}. We see that compatibility error decreases with the increase in the number of links as this drives the use of more frequencies, and also the error decreases with the increase in D, since it expands the area for compatibility computation causing more devices to be considered in a compatiblity analysis. The results indicate that based on the sensitivity of the new device/receiver, that is trying to operate in the area, an appropriate D parameter should be selected.

\begin{figure}[ht]
    \vspace{-3mm}
    \centering
    \centerline{\includegraphics[width=0.9\columnwidth]{images/sd_opt_freq.png}}
\caption{Histogram of number of channels used - SD optimization vs. Algorithm~\ref{algo:1} (100 links \& 100 trials)}
    \label{fig:sd_opt_freq}
    \vspace{-3mm}
\end{figure}

==> src/simulation_part1.tex <==
%Results from simulations that use SCMs to deconflict spectrum use between a large number of devices.
%Focus on performance measures related to spectrum use: How many channels to deconflict spectrum use. Mention that future work will try to reduce the number of channels further but the declarative nature of SCMs is a key asset to the process.
% In this section, we develop an enhanced SCM-based DSA algorithm that can deconflict the spectrum use of networks with a large number of RF devices. The algorithm leverages SCMs in a series of spectrum use compatibility computations and message exchanges to dynamically determine the transmission parameters of devices, in particular their central frequency and transmission power levels, in order to achieve \emph{aggregate compatibility}. %Additional details about the algorithm are discussed in Section~\ref{algo}. 
% Each network composed of a single transmitter-receiver pair has a designated wireless domain (WD) controller, which can interact with other WD controllers. For the exchange of SCM-based messages between WD controllers, a modified version of the Collaborative Interaction Language (CIL)~\cite{stojadinovicspectrum} developed for DARPA SC2 can be leveraged to enable information exchange. To evaluate the performance of this algorithm, we use a custom-made simulation platform described in Sec.~\ref{sim_results}. 

Allocation is responsible for carrying out the second phase of transmitter assignment after receiving a sorted list of transmitter devices. In this section, we devise a large-scale allocation strategy to license bands of spectrum to incoming transmitters in a systematic and efficient manner. Ideally, spectrum should be utilized with minimal gaps or unused spaces, ensuring that used resources are closely stacked alongside each other. The dense packing of transmitter bandwidths leaves open more continuous interval bands to meet future demand. The continuity of bandwidth intervals is necessary to accommodate future transmitters with diverse bandwidth requirements within the spectrum. Given this necessity, allocation must begin from one end of the spectrum space. Following these principles, we develop an allocation framework to capitalize on spectrum sharing opportunities, which arise with transmitter-bandwidth compatibility. We define transmitter-bandwidth compatibility as the potential for transmitters with non-interfering signals in the geographic space to share bandwidth intervals.

\begin{figure}[h]
\vspace{-4mm}
\centering
\centerline{\includegraphics[width=0.83\columnwidth]{images/allocation_plot.png}}
\vspace{-1mm}
\caption{Spectrum map showing the allocation of transmitters in defined network space (25 transmitters \& 10 bandwidth intervals).}
\label{fig:result_dsa_scheme}
\vspace{-2mm}
\end{figure}
Figure X illustrates the organization of the bandwidth space, divided into smaller resource elements and radio frames, and the use of our allocation strategy on an example set of 25 transmitters. Starting with an empty spectrum, we receive a sorted list of transmitters (\( T_{x_1}, \ldots, T_{x_{n-1}}, T_{x_n} \)), each with specific bandwidth and geographic signal requirements. Processing transmitters in the sorted order, we allocate transmitters from the leftmost endpoint of the spectrum space, moving rightward in cases of transmitter-bandwidth incompatibility. To check for compatibility at an interval, we analyze whether licensed transmitters show signal interference with the incoming transmitter. As interference is detected through geographic overlap, we consider the radii of transmitters, extending in all directions from their respective nodes, to determine any shared geographic space between them. If any licensed transmitter shares interference, the bandwidth interval is deemed incompatible and the process repeats with rightward intervals. This creates a tendency for the allocation of transmitters to flow naturally rightward across spectrum space. Overall, the left end of the spectrum exhibits a higher concentration of transmitters, indicating successful 'packing' as intended.


%For the exchange of SCM-based messages between WD controllers, we adapted a version of the Collaborative Intelligent Radio Networks (CIRN) interaction language developed by DARPA to enable information exchange between networks~\cite{sc2cil}. This language was named CIRN Interaction Language (CIL).
%In Section~\ref{platform} and ~\ref{results}, we describe the simulation platform and the results respectively. 
%The experiment described in Section~\ref{experiment} involved three networks and employed a relatively simple algorithm to coordinate the spectrum use. Taking this as a baseline, in this work we developed a more complex algorithm that uses SCMs to deconflict spectrum use between a large number of devices. The algorithm considers aggregate interference along with the option of limiting the transmission power of any new transmitter joining the system for efficient utilization of available spectrum. More details on the algorithm can be found below including simulation results in Section \ref{result}.
%
% \begin{algorithm}[!b]
% \small
% \SetAlgoLined 
% \textbf{Input:} \textit{SCMs of new and existing Tx/Rx pairs}\\ 
% \textbf{Output:} \textit{Deconflicted Tx/Rx pairs}\\
% \textbf{Initialize:} $power_{MT}$\\
% \textbf{Initialize:} $Rx_{interf} = [\ ]$\\
% \For{every new set of Tx/Rx pairs}
% {
% Get its own and existing  Tx/Rx SCMs\\
% \textbf{Initialize:} $ct\_score = 0$\\
% \textbf{Initialize:} $total_{TP} = 0$\\
% \textbf{Initialize:} $max_{PM} = 0$\\
% \For{Rx$_n$ check CT $btw$ $Tx_1..Tx_i..Tx_{n-1}$}
% {
% $total_{TP} += Tx_{inPower}$\\
% \If{\textit{compatible}}
% {
% $ct\_score += 1$
% }
% }
% \If{$ct\_score == n-1$ \textbf{and} $total_{TP} <= P_{allow Rx_n}$}
% {
% \textbf{Initialize:} $ct\_score = 0$\\
% $Rx_{interf}[n] = total_{TP}$\\
% $Tx_n\_interf = [ \ ]$\\
% \For{ Tx$_n$ check CT $btw$ $Rx_1..Rx_j..Rx_{n-1}$}
% {
%
% $Tx_n\_interf[j] = Tx_{njPower}$\\ 
% $current_{PM} = Rx_{interf}[j]+Tx_{njPower} - P_{allow Rx_j}$\\
% $max_{PM} = max(max_{PM}, current_{PM})$
%
% \If{\textit{compatible} \textbf{and} $current_{PM} <=0$}
% {
% $ct\_score += 1$
% }
% }
% \If{$ct\_score == n-1$}
% {
% \textbf{Update} $Rx_{interf} += Tx_n\_interf$
% }
% \Else{
% \If{$max_{PM} <= power_{MT}$}
% {
% \textbf{Adjust} Tx$_n$ reference power based on $max_{PM}$\\
% \textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Tx_n\_interf$
%
% \textbf{Verify} if the new link is reachable or not.
% }
% \Else{
% \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute compatibility tests
% }
% }
% }
% \Else{
% \If{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
% {
% Aggregate interference detected
% }
% \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute compatibility tests
% }
% Setup the new link\\
% Update Rx$_n$ and Tx$_n$ SCM
% }
% \caption{Spectrum Deconfliction (SD)} \label{algo:1}
% \end{algorithm}

%\vspace{-0.2cm}

% \begin{algorithm}[!b]
% \small
% \SetAlgoLined 
% \textbf{Input:} SCMs of new and existing Tx/Rx pairs\\ 
% \textbf{Output:} Deconflicted Tx/Rx pairs\\
% \textbf{Initialize:} $power_{MT}$ and $Rx_{interf} = [\ ]$\\
% \For{every new set of Tx/Rx pair}
% {
% $WD_n$ controller collects Tx/Rx SCMs\\
% \textbf{Initialize:} $ct\_score = 0$, $total_{TP} = 0$ and $max_{PM} = 0$\\
% \For{Rx$_n$ perform CT between $Tx_1..Tx_i..Tx_{n-1}$}
% {
% $total_{TP} = total_{TP} + P_{in}$\\
% \If{\textit{compatible}}
% {
% $ct\_score = ct\_score + 1$
% }
% }
% \If{$ct\_score == n-1$ \textbf{and} $total_{TP} \leq P_{allow Rx_n}$}
% {
% \textbf{Initialize:} $ct\_score = 0$ and $Rx_{interf\_n} = [ \ ]$\\
% $Rx_{interf}[n] = total_{TP}$\\
% \For{ Tx$_n$ perform CT between $Rx_1..Rx_j..Rx_{n-1}$}
% {

% $Rx_{interf\_n}[j] = P_{nj}$\\ 
% $curr_{PM} = Rx_{interf}[j]+P_{nj} - P_{allow Rx_j}$\\
% $max_{PM} = max(max_{PM}, curr_{PM})$

% \If{\textit{compatible} \textbf{and} $current_{PM} \leq 0$}
% {
% $ct\_score = ct\_score + 1$
% }
% }
% \If{$ct\_score == n-1$}
% {
% $Rx_{interf} = Rx_{interf} + Rx_{interf\_n}$
% }
% \ElseIf{$max_{PM} \leq power_{MT}$}
% {
% \textbf{Adjust} Tx$_n$ reference power based on $max_{PM}$\\
% \textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Rx_{interf\_n}$
% \textbf{Verify} if the new link is reachable or not\\
% \If{link \textbf{not} reachable}
% {
% \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute CTs
% }
% }
% \Else{
% \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute CTs
% }
% }
% \Else{
% \If{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
% {
% Aggregate interference detected
% }
% \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute CTs
% }
% Update Rx$_n$ and Tx$_n$ SCM and setup the link
% }
% \caption{Spectrum Deconfliction (SD) involving aggregate interference, frequency, and power adjustments} \label{algo:1}
% \end{algorithm}

%\subsection{Algorithm for DSA with SCMs}\label{algo}
% Our SCM-based Spectrum Deconfliction (SD) method is described in Algorithm~\ref{algo:1} with key terms defined in Table~\ref{tab:terminology}. When a new pair of devices (Tx$_n$ and Rx$_n$) enters an operational area, the SD algorithm running at the corresponding WD controller requests the SCMs of new and existing Tx and Rx pairs and then it initializes the following parameters: compatibility score ($ct\_score=0$), total power margin ($total_{PM}=0$), and maximum power margin ($max_{PM}=0$). The score is increased every time a new Tx or Rx under evaluation is determined to be compatible with a pre-existing RF counterpart (Tx vs. Rx, or, Rx vs. Tx) and is used to verify the compatibility of a new Tx/Rx pair with the entire system whereas the power margins are used to verify whether small adjustments in the power level %used in cases where we can determine that a small adjustment to the power 
% of the new transmitter (Tx$_n$) can make it compatible with existing receivers. 

% As the WD controller performs CTs between the new Rx$_n$ and existing transmitters (Tx$_1$,\ldots,Tx$_{n-1}$), if there is compatibility, the WD controller computes and updates the total aggregate interference ($total_{TP}$) at Rx$_n$. With the total aggregate interference value an aggregate evaluation of compatibility is performed. If Rx$_n$ is not compatible with the existing transmitters, i.e., if the $total_{TP}$ is greater than the allowable interference power at Rx$_n$ (identified as $P_{allow Rx_n}$), the Tx/Rx pair is moved to a different frequency channel and the CTs start over.  More details on the frequency assignment scheme will be discussed later. 
% On the other hand, if Rx$_n$ is compatible with the existing transmitters, the WD controller verifies whether Tx$_n$ is compatible with the existing receivers (Rx$_1$,\ldots,Rx$_{n-1}$). To that end, it computes the interference caused by Tx$_n$ at the existing receivers and compares it with $max_{PM}$. If Tx$_n$ is compatible with the existing receivers, the WD controller sets up the new link and updates the contribution of this new transmitter to the aggregate interference seen by each receiver using the matrix ($Rx_{interf}$). Otherwise, the WD controller attempts to achieve compatibility by decreasing Tx$_n$'s power by no more than the value of a previously agreed upon power margin threshold ($power_{MT}$). In case the power adjustment fails to achieve compatibility, the WD controller chooses a different frequency channel for the Tx/Rx pair and the CTs start over. At the end of the algorithm, once aggregate compatibility is achieved, the WD controller sets up the link and updates the SCMs of Tx$_n$ and Rx$_n$ based on the frequency and power values found to achieve global (scenario wide) compatibility so that they are ready for future CTs. %The complete procedure is described in Algorithm~\ref{algo:1} with key terms defined in Table~\ref{tab:terminology}.

% Regarding frequency assignment: Upon entering the operational area, all RF devices start with a default center frequency $f_c$ and, if needed, they move to new frequencies in $\Delta f$ increments %, based on the results of the compatibility computations, 
% until a compatible frequency for the operation of the new Tx/Rx pair is found. The objective here is to achieve high spectrum efficiency by minimizing the number of different frequency channels used. Thus, other approaches to determining  $f_c$ and $\Delta f$ can be used, but they are left for future research.  

% \begin{table}[h]
% \centering
% \small
% \caption{Key Parameters of Algorithm~\ref{algo:1}}%\igor{This is more a matter of style, but (for me) this looks slightly better. The original is commented.}}
% \vspace{-0.2cm}
% \begin{tabular}{ll}
% \toprule
% \textbf{Parameter} & \textbf{Description} \\ \midrule
% $P_{ij}$    & Interference power at j\textsuperscript{th} RX from i\textsuperscript{th} TX \\
% $Rx_{interf}$    & Interference at each RX from all existing TXs \\
% $Rx_{interf\_n}$ & Interference at each RX from TX$_n$  \\ 
% $total_{TP}$    & Total power at RX$_n$ from all existing TXs\\
% $power_{MT}$       & Power margin threshold (PMT)       \\
% $max_{PM}$ & Max power margin from all RXs                 \\ 
% $curr_{PM}$ & Current power margin          \\ 
% $P_{allow Rx_n}$ & Allowable power at RX$_n$                \\
% %$C.T.$ & Compatibility Test                \\ 
% \bottomrule
% \end{tabular}
% \label{tab:terminology}
% \vspace{-2mm}
% \end{table}

% \iffalse
% \begin{algorithm}
%  \caption{Spectrum Deconfliction (SD) Mechanism}
%  \label{algo:1}
%  \begin{algorithmic}[1]
%  \State \textbf{Input:} \textit{SCMs of new and existing Tx/Rx pairs} 
%   \State \textbf{Output:} \textit{Deconflicted Tx/Rx pairs}
%   \State \textbf{Initialize:} $power_{MT}$
%   \State \textbf{Initialize:} $Rx_{interf} = [\ ]$
% \For{every new set of Tx/Rx pairs}
%   \State Get its own and existing  Tx/Rx SCMs
%     \State \textbf{Initialize:} $ct\_score = 0$
%     \State \textbf{Initialize:} $total_{TP} = 0$
%     \State \textbf{Initialize:} $max_{PM} = 0$
%     \For{Rx$_n$ check CT $btw$ $Tx_1..Tx_i..Tx_{n-1}$}
%     \State $total_{TP} += Tx_{inPower}$
%     \If{\textit{compatible}}
%     \State$ct\_score += 1$
%      \EndIf
%     \EndFor
% \If{$ct\_score == n-1$ \textbf{and} $total_{TP} <= P_{allow Rx_n}$}
% \State \textbf{Initialize:} $ct\_score = 0$
% \State $Rx_{interf}[n] = total_{TP}$
% \State $Tx_n\_interf = [ \ ]$
% \For{ Tx$_n$ check CT $btw$ $Rx_1..Rx_j..Rx_{n-1}$}
% \If{\textit{compatible}}
%     \State$ct\_score += 1$
%      \EndIf
%     \State $Tx_n\_interf[j] = Tx_{njPower}$ 
% \State $current_{PM} = $ \\ $Rx_{interf}[j]+Tx_{njPower} - P_{allow Rx_j}$
% \State $max_{PM} = max(max_{PM}, current_{PM})$
% \EndFor
% \If{$ct\_score == n-1$}
% \State \textbf{Update} $Rx_{interf} += Tx_n\_interf$
% \Else
% \If{{$max_{PM} <= power_{MT}$}}
% \State \textbf{Adjust} Tx$_n$ reference power based on $max_{PM}$
% \State \textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Tx_n\_interf$
% \Else
% \State \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute compatibility tests
% \EndIf
% \EndIf
% \Else
% \If{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
% \State Aggregate interference detected
% \EndIf
% \State \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute compatibility tests
% \EndIf
% \State Setup the new link
% \State Update Rx$_n$ and Tx$_n$ SCM
% \EndFor
%  \end{algorithmic}
%  \end{algorithm}
% \fi

% %\iffalse
% \begin{algorithm}
%  \caption{Spectrum Deconfliction (SD)}
%  \label{algo:1}
%  \begin{algorithmic}[1]
%  \STATE \textbf{Input:} \textit{SCMs of new and existing Tx/Rx pairs}\; 
%   \STATE \textbf{Output:} \textit{Deconflicted Tx/Rx pairs}\;
%   \STATE \textbf{Initialize:} $power_{MT}$\;
%   \STATE \textbf{Initialize:} $Rx_{interf} = [\ ]$\;
% \FOR{every new set of Tx/Rx pairs}
%   \STATE Get its own and existing  Tx/Rx SCMs
%     \STATE \textbf{Initialize:} $ct\_score = 0$
%     \STATE \textbf{Initialize:} $total_{TP} = 0$
%     \STATE \textbf{Initialize:} $max_{PM} = 0$
%     \FOR{Rx$_n$ check CT $btw$ $Tx_1..Tx_i..Tx_{n-1}$}
%     \STATE $total_{TP} += Tx_{inPower}$
%     \IF{\textit{compatible}}
%     \STATE$ct\_score += 1$
%      \ENDIF
%     \ENDFOR
% \IF{$ct\_score == n-1$ \textbf{and} $total_{TP} <= P_{allow Rx_n}$}
% \STATE \textbf{Initialize:} $ct\_score = 0$
% \STATE $Rx_{interf}[n] = total_{TP}$
% \STATE $Tx_n\_interf = [ \ ]$
% \FOR{ Tx$_n$ check CT $btw$ $Rx_1..Rx_j..Rx_{n-1}$}
% \IF{\textit{compatible}}
%     \STATE$ct\_score += 1$
%      \ENDIF
%     \STATE $Tx_n\_interf[j] = Tx_{njPower}$ 
% \STATE $current_{PM} = $ \\ $Rx_{interf}[j]+Tx_{njPower} - P_{allow Rx_j}$
% \STATE $max_{PM} = max(max_{PM}, current_{PM})$
% \ENDFOR
% \IF{$ct\_score == n-1$}
% \STATE \textbf{Update} $Rx_{interf} += Tx_n\_interf$
% \ELSE
% \IF{{$max_{PM} <= power_{MT}$}}
% \STATE \textbf{Adjust} Tx$_n$ reference power based on $max_{PM}$
% \STATE \textbf{Update} $Rx_{interf}$ based on $max_{PM}$ and $Tx_n\_interf$
% \ELSE
% \STATE \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute compatibility tests
% \ENDIF
% \ENDIF
% \ELSE
% \IF{$total_{TP} > P_{allow Rx_n}$ \textbf{and} $ct\_score == n-1$}
% \STATE Aggregate interference detected
% \ENDIF
% \STATE \textbf{Change} Rx$_n$ and Tx$_n$ \underline{frequency} and recompute compatibility tests
% \ENDIF
% \STATE Setup the new link
% \STATE Update Rx$_n$ and Tx$_n$ SCM
% \ENDFOR
%  \end{algorithmic}
%  \end{algorithm}
% %\f
